Shape and Symmetry Induction for 3D Objects

Actions as simple as grasping an object or navigating around it require a rich understanding of that object's 3D shape from a given viewpoint. In this paper we repurpose powerful learning machinery, originally developed for object classification, to discover image cues relevant for recovering the 3D shape of potentially unfamiliar objects. We cast the problem as one of local prediction of surface normals and global detection of 3D reflection symmetry planes, which open the door for extrapolating occluded surfaces from visible ones. We demonstrate that our method is able to recover accurate 3D shape information for classes of objects it was not trained on, in both synthetic and real images.

==> fig1.tex <==
%\begin{figure*}
%\includegraphics[height = 1.65in]{figures/nyuIm330.png}
%\hfill
%\includegraphics[height = 1.65in]{figures/nyuIm330segOverlay.png}
%\hfill
%\includegraphics[height = 1.65in]{figures/nyuIm330Recons.png}
% \caption{ Fig 1. }
%  \figlabel{introFig}
%\end{figure*}

\twocolumn[{\begin{figure}[H]
\setlength{\linewidth}{\textwidth}
\setlength{\hsize}{\textwidth}
\centering
\includegraphics[height = 1.65in]{figures/nyuIm330.png}
\hfill
\includegraphics[height = 1.65in]{figures/nyuIm330segOverlay.png}
\hfill
\includegraphics[height = 1.65in]{figures/nyuIm330Recons.png}
 \caption{ Fig 1. }
  \figlabel{introFig}
\end{figure}}]

==> poseFigs.tex <==
\begin{figure*}[tb]
\includegraphics[width=0.97\textwidth]{figures/recog_to_recons/vpsResults.png} 
\caption{Viewpoint predictions for unoccluded groundtruth instances using our algorithm.  The columns show 15th, 30th, 45th, 60th, 75th and 90th percentile instances respectively in terms of the error. We visualize the predictions by rendering a 3D model using our predicted viewpoint.}
\figlabel{viewpointPreds}
\end{figure*}

\newcommand{\gtViewWidth}{0.186}
\newcommand{\gtViewFormat}{png}
\begin{figure*}[tb]
\centering
\setlength{\tabcolsep}{1.8pt}
\renewcommand{\arraystretch}{2.0}
\begin{tabular}{ccccc}
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/fox/1.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/fox/2.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/fox/3.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/fox/4.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/fox/5.\gtViewFormat} \\
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/golfcart/1.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/golfcart/2.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/golfcart/3.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/golfcart/4.\gtViewFormat} &
\includegraphics[width=\gtViewWidth\textwidth]{figures/poseClustersOpt/golfcart/5.\gtViewFormat}
\end{tabular}
\caption{Viewpoint predictions for novel object classes without any pose annotations. The columns show randomly selected instances whose azimuth is predicted to be around $\frac{-\pi}{2} (\text{right-facing}), \frac{-\pi}{4}, 0(\text{front-facing}), \frac{\pi}{4}, \frac{-\pi}{2}(\text{left-facing})$ respectively.}
\figlabel{inductionPreds}
\end{figure*}
